ByteTrackV2: 2D and 3D Multi-Object Tracking by Associating Every Detection Box

Multi-object tracking (MOT) aims at estimating bounding boxes and identities of objects across video frames. Detection boxes serve as the basis of both 2D and 3D MOT. The inevitable changing of detection scores leads to object missing after tracking. We propose a hierarchical data association strategy to mine the true objects in low-score detection boxes, which alleviates the problems of object missing and fragmented trajectories. The simple and generic data association strategy shows effectiveness under both 2D and 3D settings. In 3D scenarios, it is much easier for the tracker to predict object velocities in the world coordinate. We propose a complementary motion prediction strategy that incorporates the detected velocities with a Kalman filter to address the problem of abrupt motion and short-term disappearing. ByteTrackV2 leads the nuScenes 3D MOT leaderboard in both camera (56.4% AMOTA) and LiDAR (70.1% AMOTA) modalities. Furthermore, it is nonparametric and can be integrated with various detectors, making it appealing in real applications. The source code is released at https://github.com/ifzhang/ByteTrack-V2.

==> tables/app.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l c c l l c c l }

\toprule
Method & Similarity & BYTE & MOTA$\uparrow$ & IDF1$\uparrow$ & IDs$\downarrow$\\
\midrule
JDE \cite{wang2020towards} & Motion(K)+Re-ID &  & 60.0 & 63.6 & 473\\
 & Motion(K)+Re-ID & $\checkmark$ & 60.3 (+0.3) & 64.1 (+0.5) & 418\\
 & Motion(K) & $\checkmark$ & 60.6 (+0.6) & 66.0 \textcolor{codegreen}{(+\textbf{2.4})} & 360\\

\midrule
CSTrack \cite{liang2020rethinking} & Motion(K)+Re-ID &  & 68.0 & 72.3 & 325\\
 & Motion(K)+Re-ID & $\checkmark$ & 69.2 \textcolor{codegreen}{(+\textbf{1.2})} & 73.9 \textcolor{codegreen}{(+\textbf{1.6})} & 285\\
 & Motion(K) & $\checkmark$ & 69.3 \textcolor{codegreen}{(+\textbf{1.3})} & 71.7 (-0.6) & 279\\

\midrule
FairMOT \cite{zhang2020fairmot} & Motion(K)+Re-ID &  & 69.1 & 72.8 & 299\\
 & Motion(K)+Re-ID & $\checkmark$ & 70.4 \textcolor{codegreen}{(+\textbf{1.3})} & 74.2 \textcolor{codegreen}{(+\textbf{1.4})} & 232\\
 & Motion(K) & $\checkmark$ & 70.3 \textcolor{codegreen}{(+\textbf{1.2})} & 73.2 (+0.4) & 236\\
 
\midrule
TraDes \cite{wu2021track} & Motion+Re-ID &  & 68.2 & 71.7 & 285\\
 & Motion+Re-ID & $\checkmark$ & 68.6 (+0.4) & 71.1 (-0.6) & 259\\
 & Motion(K) & $\checkmark$ & 67.9 (-0.3) & 72.0 (+0.3) & 178\\

\midrule
QDTrack \cite{pang2021quasi} & Re-ID & & 67.3 & 67.8 & 377\\
& Motion(K)+Re-ID & $\checkmark$ & 67.7 (+0.4) & 72.0 \textcolor{codegreen}{(+\textbf{4.2})} & 281\\
& Motion(K) & $\checkmark$ & 67.9  (+0.6) & 70.9  \textcolor{codegreen}{(+\textbf{3.1})} & 258\\
 
\midrule
CenterTrack \cite{zhou2020tracking} & Motion &  & 66.1 & 64.2 & 528\\
 & Motion & $\checkmark$ & 66.3 (+0.2) & 64.8 (+0.6) & 334\\
 & Motion(K) & $\checkmark$ & 67.4 \textcolor{codegreen}{(+\textbf{1.3})} & 74.0 \textcolor{codegreen}{(+\textbf{9.8})} & 144\\
 
\midrule
CTracker \cite{peng2020chained} & Chain &  & 63.1 & 60.9 & 755\\
 & Motion(K) & $\checkmark$ & 65.0 \textcolor{codegreen}{(+\textbf{1.9})} & 66.7 \textcolor{codegreen}{(+\textbf{5.8})} & 346\\

\midrule
TransTrack \cite{sun2020transtrack} & Attention &  & 67.1 & 68.3 & 254\\
 & Attention & $\checkmark$ & 68.6 \textcolor{codegreen}{(+\textbf{1.5})} & 69.0 (+0.7) & 232\\
 & Motion(K) & $\checkmark$ & 68.3 \textcolor{codegreen}{(+\textbf{1.2})}& 72.4  \textcolor{codegreen}{(+\textbf{4.1})} & 181\\
 
\midrule
MOTR \cite{zeng2021motr} & Attention &  & 64.7 & 67.2 & 346\\
 & Attention & $\checkmark$ & 64.3 (-0.4) & 69.3 \textcolor{codegreen}{(+\textbf{2.1})} & 263\\
 & Motion(K) & $\checkmark$ & 65.7 \textcolor{codegreen}{(+\textbf{1.0})} & 68.4 \textcolor{codegreen}{(+\textbf{1.2})} & 260\\
\bottomrule
\end{tabular}

==> tables/app_all.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c c | l l c c l }

\toprule
Method & Similarity & w/ BYTE & MOTA$\uparrow$ & IDF1$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDs$\downarrow$\\
\midrule
JDE \cite{wang2020towards} & Motion(K) + Re-ID &  & 60.0 & 63.6 & 2923 & 18158 & 473\\
 & Motion(K) + Re-ID & $\checkmark$ & 60.3 (+0.3) & 64.1 (+0.5) & 3065 & 17912 & 418\\
 & Motion(K) & $\checkmark$ & 60.6 (+0.6) & 66.0 \textcolor{codegreen}{(+\textbf{2.4})} & 3082 & 17771 & 360\\

\midrule
CSTrack \cite{liang2020rethinking} & Motion(K) + Re-ID &  & 68.0 & 72.3 & 1846 & 15075 & 325\\
 & Motion(K) + Re-ID & $\checkmark$ & 69.2 \textcolor{codegreen}{(+\textbf{1.2})} & 73.9 \textcolor{codegreen}{(+\textbf{1.6})} & 2160 & 14128 & 285\\
 & Motion(K) & $\checkmark$ & 69.3 \textcolor{codegreen}{(+\textbf{1.3})} & 71.7 (-0.6) & 2202 & 14068 & 279\\

\midrule
FairMOT \cite{zhang2020fairmot} & Motion(K) + Re-ID &  & 69.1 & 72.8 & 1976 & 14443 & 299\\
 & Motion(K) + Re-ID & $\checkmark$ & 70.4 \textcolor{codegreen}{(+\textbf{1.3})} & 74.2 \textcolor{codegreen}{(+\textbf{1.4})} & 2288 & 13470 & 232\\
 & Motion(K) & $\checkmark$ & 70.3 \textcolor{codegreen}{(+\textbf{1.2})} & 73.2 (+0.4) & 2189 & 13625 & 236\\
 
\midrule
TraDes \cite{wu2021track} & Motion + Re-ID &  & 68.2 & 71.7 & 1913 & 14962 & 285\\
 & Motion + Re-ID & $\checkmark$ & 68.6 (+0.4) & 71.1 (-0.6) & 2253 & 14419 & 259\\
 & Motion(K) & $\checkmark$ & 67.9 (-0.3) & 72.0 (+0.3) & 1822 & 15345 & 178\\

\midrule
QDTrack \cite{pang2021quasi} & Re-ID & & 67.3 & 67.8 & 2637 & 14605 & 377\\
& Motion(K) + Re-ID & $\checkmark$ & 67.7 (+0.4) & 72.0 \textcolor{codegreen}{(+\textbf{4.2})} & 2280 & 14856 & 281\\
& Motion(K) & $\checkmark$ & 67.9  (+0.6) & 70.9  \textcolor{codegreen}{(+\textbf{3.1})} & 2310 & 14746 & 258\\
 
\midrule
CenterTrack \cite{zhou2020tracking} & Motion &  & 66.1 & 64.2 & 2442 & 15286 & 528\\
 & Motion & $\checkmark$ & 66.3 (+0.2)  & 64.8 (+0.6)  & 2376 & 15445 & 334\\
 & Motion(K) & $\checkmark$ & 67.4 \textcolor{codegreen}{(+\textbf{1.3})} & 74.0 \textcolor{codegreen}{(+\textbf{9.8})} & 1778 & 15641 & 144\\
 
\midrule
CTracker \cite{peng2020chained} & Chain &  & 63.1 & 60.9 & 2955 & 16174 & 755\\
 & Motion(K) & $\checkmark$ & 65.0 \textcolor{codegreen}{(+\textbf{1.9})} & 66.7 \textcolor{codegreen}{(+\textbf{5.8})} & 3303 & 15206 & 346\\

\midrule
TransTrack \cite{sun2020transtrack} & Attention &  & 67.1 & 68.3 & 1652 & 15817 & 254\\
 & Attention & $\checkmark$ & 68.6 \textcolor{codegreen}{(+\textbf{1.5})} & 69.0 (+0.7) & 2151 & 14515 & 232\\
 & Motion(K) & $\checkmark$ & 68.3 \textcolor{codegreen}{(+\textbf{1.2})}& 72.4  \textcolor{codegreen}{(+\textbf{4.1})} & 1692 & 15189 & 181\\
 
\midrule
MOTR \cite{zeng2021motr} & Attention &  & 64.7 & 67.2 & 5278 & 13452 & 346\\
 & Attention & $\checkmark$ & 64.3 (-0.4) & 69.3 \textcolor{codegreen}{(+\textbf{2.1})} & 5787 & 13220 & 263\\
 & Motion(K) & $\checkmark$ & 65.7 \textcolor{codegreen}{(+\textbf{1.0})} & 68.4 \textcolor{codegreen}{(+\textbf{1.2})} & 1607 & 16651 & 260\\
\bottomrule
\end{tabular}

==> tables/input_size.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c c c c}

\toprule
Input size & MOTA$\uparrow$ & IDF1$\uparrow$ & IDs$\downarrow$ & Time (ms) \\
\midrule
$512 \times 928$ & 75.0 & 77.6 & 200 & \textbf{17.9+4.0}\\
$608 \times 1088$ & 75.6 & 76.4 & 212 & 21.8+4.0\\
$736 \times 1280$ & 76.2 & 77.4 & 188 & 26.2+4.2\\
$800 \times 1440$ & \textbf{76.6} & \textbf{79.3} & \textbf{159} & 29.6+4.2 \\
\bottomrule
\end{tabular}

==> tables/inter.tex <==
\setlength{\tabcolsep}{8.0pt}

\begin{tabular}{ c c c c c c c}

\toprule
Interval & MOTA$\uparrow$ & IDF1$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDs$\downarrow$\\
\midrule
No & 76.6 & 79.3 & \textbf{3358} & 9081 & 159\\
10 & 77.4 & 79.7 & 3638 & 8403 & 150\\
20 & \textbf{78.3} & \textbf{80.2} & 3941 & 7606 & \textbf{146}\\
30 & 78.3 & 80.2 & 4237 & \textbf{7337} & 147\\
\bottomrule
\end{tabular}

==> tables/light.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l c c | l c c c}

\toprule
Backbone & Params & GFLOPs & Tracker & MOTA$\uparrow$ & IDF1$\uparrow$ & IDs$\downarrow$ \\
\midrule
YOLOX-M & 25.3 M & 118.7 & DeepSORT & 74.5 & 76.2 & 197\\
YOLOX-M & 25.3 M & 118.7 & BYTE & 75.3 & 77.5 & 200\\
YOLOX-S & 8.9 M & 43.0 & DeepSORT & 69.6 & 71.5 & 205\\
YOLOX-S & 8.9 M & 43.0 & BYTE & 71.1 & 73.6 & 224\\
YOLOX-Tiny & 5.0 M & 24.5 & DeepSORT & 68.6 & 72.0 & 224\\
YOLOX-Tiny & 5.0 M & 24.5 & BYTE & 70.5 & 72.1 & 222\\
YOLOX-Nano & 0.9 M & 4.0 & DeepSORT & 61.4 & 66.8 & 212\\
YOLOX-Nano & 0.9 M & 4.0 & BYTE & 64.4 & 68.4 & 161\\
\bottomrule
\end{tabular}

==> tables/mot17_all.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c c c c c c c c c}

\toprule
Tracker & MOTA$\uparrow$ & IDF1$\uparrow$ & HOTA$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDs$\downarrow$ & FPS$\uparrow$\\
\midrule
DAN \cite{sun2019deep} & 52.4 & 49.5 & 39.3 & 21.4\% & 30.7\% & 25423 & 234592 & 8431 & \textless 3.9\\ 
Tube\_TK \cite{pang2020tubetk} & 63.0 & 58.6 & 48.0 & 31.2\% & 19.9\% & 27060 & 177483 & 4137 & 3.0\\
MOTR \cite{zeng2021motr} & 65.1 & 66.4 & - & 33.0\% & 25.2\% & 45486 & 149307 & 2049 & -\\
CTracker \cite{peng2020chained} & 66.6 & 57.4 & 49.0 & 37.8\% & 18.5\% & 22284 & 160491 & 5529 & 6.8\\
CenterTrack \cite{zhou2020tracking} & 67.8 & 64.7 & 52.2 & 34.6\% & 24.6\% & \textbf{18498} & 160332 & 3039 & 17.5\\
QuasiDense \cite{pang2021quasi} & 68.7 & 66.3 & 53.9 & 40.6\% & 21.9\% & 26589 & 146643 & 3378 & 20.3\\
TraDes \cite{wu2021track} & 69.1 & 63.9 & 52.7 & 36.4\% & 21.5\% & 20892 & 150060 & 3555 & 17.5\\
MAT \cite{han2020mat} & 69.5 & 63.1 & 53.8 & 43.8\% & 18.9\% & 30660 & 138741 & 2844 & 9.0\\
SOTMOT \cite{zheng2021improving} & 71.0 & 71.9 & - & 42.7\% & 15.3\% & 39537 & 118983 & 5184 & 16.0\\
TransCenter \cite{xu2021transcenter} & 73.2 & 62.2 & 54.5 & 40.8\% & 18.5\% & 23112 & 123738 & 4614 & 1.0\\
GSDT \cite{wang2020joint} & 73.2 & 66.5 & 55.2 & 41.7\% & 17.5\% & 26397 & 120666 & 3891 & 4.9\\
Semi-TCL \cite{li2021semi} & 73.3 & 73.2 & 59.8 & 41.8\% & 18.7\% & 22944 & 124980 & 2790 & -\\
FairMOT \cite{zhang2020fairmot} & 73.7 & 72.3 & 59.3 & 43.2\% & 17.3\% & 27507 & 117477 & 3303 & 25.9\\
RelationTrack \cite{yu2021relationtrack} & 73.8 & 74.7 & 61.0 & 41.7\% & 23.2\% & 27999 & 118623 & \textbf{1374} & 8.5\\
PermaTrackPr \cite{tokmakov2021learning} & 73.8 & 68.9 & 55.5 & 43.8\% & 17.2\% & 28998 & 115104 & 3699 & 11.9\\
CSTrack \cite{liang2020rethinking} & 74.9 & 72.6 & 59.3 & 41.5\% & 17.5\% & 23847 & 114303 & 3567 & 15.8\\
TransTrack \cite{sun2020transtrack} & 75.2 & 63.5 & 54.1 & \textbf{55.3\%} & \textbf{10.2\%} & 50157 & 86442 & 3603 & 10.0\\
FUFET \cite{shan2020tracklets} & 76.2 & 68.0 & 57.9 & 51.1\% & 13.6\% & 32796 & 98475 & 3237 & 6.8\\
SiamMOT \cite{liang2021one} & 76.3 & 72.3 & - & 44.8\% & 15.5\% & - & - & - & 12.8\\
CorrTracker \cite{wang2021multiple} & 76.5 & 73.6 & 60.7 & 47.6\% & 12.7\% & 29808 & 99510 & 3369 & 15.6\\
TransMOT \cite{chu2021transmot} & 76.7 & 75.1 & 61.7 & 51.0\% & 16.4\% & 36231 & 93150 & 2346 & 9.6\\
ReMOT \cite{yang2021remot} & 77.0 & 72.0 & 59.7 & 51.7\% & 13.8\% & 33204 & 93612 & 2853 & 1.8\\
\textbf{ByteTrack (ours)} & \textbf{80.3} & \textbf{77.3} & \textbf{63.1} & 53.2\% & 14.5\% & 25491 & \textbf{83721} & 2196 & \textbf{29.6}\\
\bottomrule
\end{tabular}

==> tables/mot17_pub.tex <==
\setlength{\tabcolsep}{3.0pt}

\begin{tabular}{ l c c c c c c}

\toprule
Tracker & MOTA$\uparrow$ & IDF1$\uparrow$ & HOTA$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDs$\downarrow$\\
\midrule
STRN \cite{xu2019spatial} & 50.9 & 56.0 & 42.6 & 25295 & 249365 & 2397\\
FAMNet \cite{chu2019famnet} & 52.0 & 48.7 & - & 14138 & 253616 & 3072\\
Tracktor++v2 \cite{bergmann2019tracking} & 56.3 & 55.1 & 44.8 & \textbf{8866} & 235449 & 1987\\
MPNTrack \cite{braso2020learning} & 58.8 & 61.7 & 49.0 & 17413 & 213594 & 1185\\
LPC\_MOT \cite{dai2021learning} & 59.0 & 66.8 & 51.5 & 23102 & 206948 & \textbf{1122}\\
Lif\_T \cite{hornakova2020lifted} & 60.5 & 65.6 & 51.1 & 14966 & 206619 & 1189\\
CenterTrack \cite{zhou2020tracking} & 61.5 & 59.6 & 48.2 & 14076 & 200672 & 2583\\
TMOH \cite{stadler2021improving} & 62.1 & 62.8 & 50.4 & 10951 & 201195 & 1897\\
ArTIST\_C \cite{saleh2021probabilistic} & 62.3 & 59.7 & 48.9 & 19611 & 191207 & 2062\\
QDTrack \cite{pang2021quasi} & 64.6 & 65.1 & - & 14103 & 182998 & 2652\\
SiamMOT \cite{shuai2021siammot} & 65.9 & 63.3 & - & 18098 & 170955 & 3040\\
\cellcolor{Gray}ByteTrack-2D & \cellcolor{Gray}\textbf{67.4} & \cellcolor{Gray}\textbf{70.0} & \cellcolor{Gray}\textbf{56.1} & \cellcolor{Gray}9939 & \cellcolor{Gray}\textbf{172636} & \cellcolor{Gray}1331\\
\bottomrule
\end{tabular}

==> tables/mot20_all.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c c c c c c c c c}

\toprule
Tracker & MOTA$\uparrow$ & IDF1$\uparrow$ & HOTA$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDs$\downarrow$ & FPS$\uparrow$\\
\midrule
MLT \cite{zhang2020multiplex} & 48.9 & 54.6 & 43.2 & 30.9\% & 22.1\% & 45660 & 216803 & 2187 & 3.7\\
FairMOT \cite{zhang2020fairmot} & 61.8 & 67.3 & 54.6 & 68.8\% & \textbf{7.6\%} & 103440 & 88901 & 5243 & 13.2\\
TransCenter \cite{xu2021transcenter} & 61.9 & 50.4 & - & 49.4\% & 15.5\% & 45895 & 146347 & 4653 & 1.0\\
TransTrack \cite{sun2020transtrack} & 65.0 & 59.4 & 48.5 & 50.1\% & 13.4\% & 27197 & 150197 & 3608 & 7.2\\
CorrTracker \cite{wang2021multiple} & 65.2 & 69.1 & - & 66.4\% & 8.9\% & 79429 & 95855 & 5183 & 8.5\\
Semi-TCL \cite{li2021semi} & 65.2 & 70.1 & 55.3 & 61.3\% & 10.5\% & 61209 & 114709 & 4139 & -\\
CSTrack \cite{liang2020rethinking} & 66.6 & 68.6 & 54.0 & 50.4\% & 15.5\% & \textbf{25404} & 144358 & 3196 & 4.5\\
GSDT \cite{wang2020joint} & 67.1 & 67.5 & 53.6 & 53.1\% & 13.2\% & 31913 & 135409 & 3131 & 0.9\\
SiamMOT \cite{liang2021one} & 67.1 & 69.1 & - & 49.0\% & 16.3\% & - & - & - & 4.3\\
RelationTrack \cite{yu2021relationtrack} & 67.2 & 70.5 & 56.5 & 62.2\% & 8.9\% & 61134 & 104597 & 4243 & 2.7\\
SOTMOT \cite{zheng2021improving} & 68.6 & 71.4 & - & 64.9\% & 9.7\% & 57064 & 101154 & 4209 & 8.5\\
\textbf{ByteTrack (ours)} & \textbf{77.8} & \textbf{75.2} & \textbf{61.3} & \textbf{69.2\%} & 9.5\% & 26249 & \textbf{87594} & \textbf{1223} & \textbf{17.5}\\
\bottomrule
\end{tabular}

==> tables/mot20_pub.tex <==
\setlength{\tabcolsep}{3.0pt}

\begin{tabular}{ l c c c c c c}

\toprule
Tracker & MOTA$\uparrow$ & IDF1$\uparrow$ & HOTA$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDs$\downarrow$\\
\midrule
SORT \cite{bewley2016simple} & 42.7 & 45.1 & 36.1 & 27521 & 264694 & 4470\\
Tracktor++v2 \cite{bergmann2019tracking} & 52.6 & 52.7 & 42.1 & \textbf{6930} & 236680 & 1648\\
ArTIST\_C \cite{saleh2021probabilistic} & 53.6 & 51.0 & 41.6 & 7765 & 230576 & 1531\\
LPC\_MOT \cite{dai2021learning} & 56.3 & 62.5 & 49.0 & 11726 & 213056 & 1562\\
MPNTrack \cite{braso2020learning} & 57.6 & 59.1 & 46.8 & 16953 & 201384 & 1210\\
TMOH \cite{stadler2021improving} & 60.1 & 61.2 & 48.9 & 38043 & 165899 & 2342\\
\cellcolor{Gray}ByteTrack-2D & \cellcolor{Gray}\textbf{67.0} & \cellcolor{Gray}\textbf{70.2} & \cellcolor{Gray}\textbf{56.4} & \cellcolor{Gray}9685 & \cellcolor{Gray}\textbf{160303} & \cellcolor{Gray}\textbf{680}\\
\bottomrule
\end{tabular}

==> tables/motion.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c c c c c}

\toprule
Prediction & w/ low-score & MOTA$\uparrow$ & IDF1$\uparrow$ & IDs$\downarrow$ & FPS \\
\midrule
K=5 &  & 74.6 & 76.9 & 291 & \textbf{30.1}\\
K=10 &  & 75.4 & 77.2 & 239 & 13.5\\
K=20 &  & 75.4 & 77.6 & 247 & 11.1\\
\textbf{BYTE (ours)} & $\checkmark$ & \textbf{76.6} & \textbf{79.3} & \textbf{159} & 29.2 \\
\bottomrule
\end{tabular}

==> tables/reid.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c c | c c c}

\toprule
Method & Similarity\#1 & Similarity\#2 & MOTA$\uparrow$ & IDF1$\uparrow$ & IDs$\downarrow$\\
\midrule
FairMOT \cite{zhang2020fairmot} & Re-ID & Re-ID & 69.8 & \textbf{74.2} & 279\\
 & Re-ID & IoU & \textbf{70.4} & \textbf{74.2} & \textbf{232}\\
\midrule
ByteTrack & IoU & Re-ID & 75.8 & 77.5 & 231 \\
 & IoU & IoU & \textbf{76.6} & 79.3 & \textbf{159}\\
 & Re-ID & Re-ID & 75.2 & 78.7 & 276\\
 & Re-ID & IoU & 76.3 & \textbf{80.5} & 216\\
\bottomrule
\end{tabular}

==> tables/training_data.tex <==
\setlength{\tabcolsep}{1.0pt}

\begin{tabular}{ l | c | c c c}

\toprule
Training data & Images & MOTA$\uparrow$ & IDF1$\uparrow$ & IDs$\downarrow$\\
\midrule
MOT17 & 2.7K & 75.8 & 76.5 & 205\\
MOT17 + CH & 22.0K & 76.6 & 79.3 & \textbf{159}\\
MOT17 + CH + CE & 26.6K & \textbf{76.7} & \textbf{79.7} & 183 \\
\bottomrule
\end{tabular}
